Unifying the Discrete and Continuous Emotion labels for Speech Emotion Recognition

Traditionally, in paralinguistic analysis for emotion detection from speech, emotions have been identified with discrete or dimensional (continuous-valued) labels. Accordingly, models that have been proposed for emotion detection use one or the other of these label types. However, psychologists like Russell and Plutchik have proposed theories and models that unite these views, maintaining that these representations have shared and complementary information. This paper is an attempt to validate these viewpoints computationally. To this end, we propose a model to jointly predict continuous and discrete emotional attributes and show how the relationship between these can be utilized to improve the robustness and performance of emotion recognition tasks. Our approach comprises multi-task and hierarchical multi-task learning frameworks that jointly model the relationships between continuous-valued and discrete emotion labels. Experimental results on two widely used datasets (IEMOCAP and MSPPodcast) for speech-based emotion recognition show that our model results in statistically significant improvements in performance over strong baselines with non-unified approaches. We also demonstrate that using one type of label (discrete or continuous-valued) for training improves recognition performance in tasks that use the other type of label. Experimental results and reasoning for this approach (called the mismatched training approach) are also presented.

==> sections/setup.tex <==
\subsection{Data}

Our experiments are conducted on the MSP podcast\cite{Lotfian_2019_3} and IEMOCAP \cite{busso2008iemocap}. MSP Podcast is the largest human labelled emotion dataset. It is comprised of segments of speech from podcasts, which means that the speech is expressive and the acoustic environment less constrained by background noise and other interference. The MSPPodcast data has labels for three continuous dimensions - valence, arousal and dominance, and for 5 discrete emotions - neutral, angry, happy, sad, and disgust. In this work, we report our results on the balanced test1 evaluation set with 30 male and 30 female speakers. IEMOCAP is total 20 hours dataset, which is acted emotion. It is labelled for three continuous dimensions - valence, arousal and dominance, and for 5 discrete emotions - neutral, angry, happy, sad, and disgust
 

\subsection{Models}
All our models are built using the ESPNet\cite{watanabe2018espnet} toolkit. Our code will be made publicly available to encourage further research in this direction. Self-supervised representation learning models are among the start of the art for many tasks including speech emotion recognition, and hence we use \texttt{HUBERT-base} as the encoder for our emotion recognition. HUBERT\cite{hsu2021hubert} is an iterative estimator with masked acoustic frame classification as the proxy task. Subsequent iterations produce different classification targets as clustering is performed on different feature sets including MFCCs and intermediate layer activations from previous iterations. The base HUBERT model comprises CNN feature extractors followed by 12 BERT-like transformer layers. We use the \texttt{HUBERT-base} model without ASR finetuning, and freeze the parameters in the CNN feature extractor while training all our models.  
We employ self-attentive pooling\cite{safari2020self} so the model can learn which frames to focus on in order to make predictions of emotion attributes. Our decoders consist of Linear projections that map from the encode output dimension 768 to 64, 32 and consequently the output sizes of 3 for the dimensional prediction and 5 for the discrete prediction.  We use a ReLU activation to ensure that the predicted continuous attributes are strictly positive and use LeakyReLU elsewhere. We use a dropout of 0.2 in the decoder. Our models are trained with the Adam optimizer, and a learning rate of 8e-5 for the encoder, and 1e-4 for the decoder. The learning rate is decayed by 0.85 when the validation score ( mean of accuracy for discrete classification and CCC metric for continuous prediction) does not improve. 

\subsection{Evaluation Metrics}
Discrete emotion recognition is evaluated using standard classification metrics like accuracy, and F-1 scores. For continuous dimension prediction, we compute the Concordance Correlation Coefficient for each of the attributes arousal, valence and dominance, and consequently their mean. Equation \eqref{eqn_ccc_metric} shows how the CCC is computed given prediction $\hat{c}$, and ground truth $c$.  

\begin{equation}
    \mathcal{L_\text{ccc}} = \dfrac{2\sigma^2{c\hat{c}}}{\sigma_{c}^2 + \sigma_{\hat{c}}^2 + (\mu_c -\mu_{\hat{c}})^2} \label{eqn_ccc_metric}
\end{equation}
